Magnetometer-free inertial motion tracking of arbitrary joints with range of motion constraints

In motion tracking of connected multi-body systems Inertial Measurement Units (IMUs) are used in a wide variety of applications, since they provide a low-cost easy-to-use method for orientation estimation. However, in indoor environments or near ferromagnetic material the magnetic field is inhomogeneous which limits the accuracy of tracking algorithms using magnetometers. Methods that use only accelerometers and gyroscopes on the other hand yield no information on the absolute heading of the tracked object. For objects connected by rotational joints with range of motion constraints we propose a method that provides a magnetometer-free, long-term stable relative orientation estimate based on a non-linear, window-based cost function. The method can be used for real-time estimation as well as post-processing. It is validated experimentally with a mechanical joint and compared to other methods that are used in motion tracking. It is shown that for the used test object, the proposed methods yields the best results with a total angle error of less than 4 degrees for all experiments.

==> macros.tex <==
%% START OF COMMAND DEFINITIONS

\makeatletter

\newlength\figH
\newlength\figW

\tikzset{
  distance from start/.code={%
    \pgfgetpath\currentpath\pgfprocessround{\currentpath}{\currentpath}%
    \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
    \pgfmathparse{#1/\pgf@decorate@totalpathlength}\tikzset{pos=\pgfmathresult}},
  distance from end/.code={%
    \pgfgetpath\currentpath\pgfprocessround{\currentpath}{\currentpath}%
    \pgf@decorate@parsesoftpath{\currentpath}{\currentpath}%
    \pgfmathparse{1-(#1/\pgf@decorate@totalpathlength)}\tikzset{pos=\pgfmathresult}}
}
\makeatother


\def\MBOLD#1%
    {\IfSubStr{ABCDEFGHIJKLMNOPQRSTUVWXYZabcdefghijklmnopqrstuvwxyz}{#1}
        {\mathbf{#1}}
        {\bm{#1}}}

\newcommand\smallminus{%
  \setbox0=\hbox{-}%
  \vcenter{%
    \hrule width\wd0 height \the\fontdimen8\textfont3%
  }%
}
\newcommand{\inksvcenter}[1]{\raisebox{-0.4\height}{#1}}
\renewcommand{\c}[1]{\raisebox{-0.3\height}{#1}}
% \renewcommand{\c}[1]{\adjustbox{raise=-0.4\height}{#1}}
% \renewcommand{\c}[1]{{\vspace{\baselineskip}#1}}
% \renewcommand{\c}[1]{{#1}}
\newcommand{\smallequal}{{\scriptstyle{=}}}
\newcommand{\se}{{\scriptstyle{=}}}

\newcommand{\fa}{\textcolor{green_gui}{a}}
\newcommand{\fb}{\textcolor{blue_gui}{b}}
\newcommand{\fc}{\textcolor{orange_gui}{c}}
\newcommand{\fd}{\textcolor{purple_gui}{d}}

\definecolor{ma_blue}{RGB}{31, 119, 179}
\definecolor{ma_green}{RGB}{43, 159, 43}
\definecolor{ma_orange}{RGB}{255, 126, 14}
\newcommand{\tb}[1]{\textcolor{ma_blue}{#1}}
\newcommand{\tg}[1]{\textcolor{ma_green}{#1}}
\renewcommand{\to}[1]{\textcolor{ma_orange}{#1}}
%% References
\newcommand{\reffig}[1]{Fig. \ref{#1}}
\newcommand{\refsection}[1]{Section \ref{#1}}
\newcommand{\refappendix}[1]{Appendix \ref{#1}}
\newcommand{\refchapter}[1]{Chapter \ref{#1}}
\newcommand{\refequation}[1]{\eqref{#1}}
\newcommand{\reftable}[1]{Table ~\ref{#1}}
\newcommand{\refeqnamed}[2]{\hyperref[#2]{#1}~\eqref{#2}}

\renewcommand{\refsection}[1]{\hyperref[#1]{Sec.} \ref{#1}}
\newcommand{\chapterref}[1]{\hyperref[#1]{Ch.} \ref{#1}}
\newcommand{\appref}[1]{\hyperref[#1]{App.} \ref{#1}}
\newcommand{\sectionref}[1]{\hyperref[#1]{Sec.} \ref{#1}}
\renewcommand{\reffig}[1]{\hyperref[#1]{Fig.} \ref{#1}}
\newcommand{\figref}[1]{\hyperref[#1]{Fig.} \ref{#1}}
\newcommand{\method}[2]{\hyperref[#2]{\textsc{#1}}~}
\newcommand{\theoremref}[1]{\hyperref[#1]{Th.} \ref{#1}}
\newcommand{\defref}[1]{\hyperref[#1]{Def.} \ref{#1}}
\newcommand{\tableref}[1]{\hyperref[#1]{Table} \ref{#1}}
\newcommand{\tabref}[1]{\hyperref[#1]{Table} \ref{#1}}
%% Notes

\newcommand{\wording}[1]{\textcolor{orange_gui}{#1}}
\newcommand{\tbd}[1]{\textcolor{purple_gui}{#1}}

%% Vecs, Quats
% \renewcommand{\vec}[2][]{\ensuremath{\coordtrafobrackets{#1}{\mathbf{#2}}}}
\renewcommand{\vec}[2][]{\ensuremath{\prescript{}{\mathcal{#1}}{\mathbf{#2}}}}
\newcommand{\quat}[3][]{\ensuremath{\coordtrafobrackets{#1}{\prescript{\frame{#2}}{\frame{#3}}{\mathbf{q}}}}}
\newcommand{\quatest}[3][]{\ensuremath{\coordtrafobrackets{#1}{\prescript{\frame{#2}}{\frame{#3}}{\hat{\mathbf{q}}}}}}
\newcommand{\quattilde}[3][]{\ensuremath{\coordtrafobrackets{#1}{\prescript{\frame{#2}}{\frame{#3}}{\tilde{\mathbf{q}}}}}}
\newcommand{\vecframe}[3]{\ensuremath{\prescript{\frame{#2}}{\frame{#3}}{\mathbf{#1}}}}

\renewcommand{\frame}[1]{\ensuremath{\mathcal{#1}}}

%% Components
\newcommand{\quatcomp}[4]{\ensuremath{\begin{bmatrix}#1 & #2 & #3 & #4 \end{bmatrix}^T}}
\newcommand{\veccomp}[3]{\ensuremath{\begin{bmatrix}#1 & #2 & #3 \end{bmatrix}^T}}
\newcommand{\veccompt}[2]{\ensuremath{\begin{bmatrix}#1 & #2\end{bmatrix}^T}}
\newcommand{\quatsin}[1]{\ensuremath{\sin\left(\frac{#1}{2}\right)}}
\newcommand{\quatcos}[1]{\ensuremath{\cos\left(\frac{#1}{2}\right)}}
\newcommand{\veccompup}[3]{\ensuremath{\begin{bmatrix}#1 \\ #2 \\ #3 \end{bmatrix}}}


\newcommand{\euler}[2]{\ensuremath{\textrm{Eu}_{\textrm{#1}}(#2)}}
\newcommand{\quateuler}[4]{\ensuremath{\textrm{Q}_{\textrm{#1}}(#2,#3,#4)}}
\newcommand{\squat}[3][]{\ensuremath{\left(\mbox{}^{#2}_{#3}\right)_{#1}}}
\newcommand{\quataa}[2]{\ensuremath{\mathrm{Q}\left(#1, #2\right)}}
\newcommand{\nvec}[3][]{\ensuremath{\coordtrafobrackets{#1}{\MBOLD{#2}_{\mathrm{#3}}}}}
\newcommand{\nquat}[2][]{\nvec[#1]{q}{#2}}
\newcommand{\coordtrafobrackets}[2]{\ifthenelse{\equal{#1}{}}{#2}{\left[#2\right]_{#1}}}

% \newcommand{\gyr}[2][]{\ensuremath{\nvec[#1]{\omega}{_{#2}}}}
% \newcommand{\acc}[2][]{\ensuremath{\nvec[#1]{\mathbf{a}}{_{#2}}}}
% \newcommand{\mmag}[2][]{\ensuremath{\nvec[#1]{\mathbf{m}}{_{#2}}}}
\newcommand{\gyr}[2][]{\ensuremath{_{\scriptscriptstyle{\frame{#1}}}{\MBOLD{\omega}}{_{#2}}}}
\newcommand{\acc}[2][]{\ensuremath{_{\scriptscriptstyle{\frame{#1}}}{\MBOLD{a}}{_{#2}}}}
\newcommand{\mmag}[2][]{\ensuremath{_{\scriptscriptstyle{\frame{#1}}}{\MBOLD{m}}{_{#2}}}}

\newcommand{\jn}{\nvec{j}{n}}
\newcommand{\ja}[1][]{{{\vec{j}}_\text{#1}}}
\newcommand{\jaskew}[2][]{\ensuremath{\vec[#1]{\tilde{j}}_\mathrm{#2}}}

\newcommand{\jaxis}[1]{\vec{j}_\mathrm{#1}}

\newcommand{\jangle}[1]{\ensuremath{\varphi_\mathrm{#1}}}

\newcommand{\samplerate}{\ensuremath{f_\mathrm{s}}}


%% Operators
\newcommand{\quatinv}{\ensuremath{^{\smallminus1}}}
\newcommand{\quatconj}{\ensuremath{^{\ast}}}
\newcommand{\quatmult}{\ensuremath{\otimes}}
\newcommand{\rot}{\ensuremath{\mathrm{R}}}
\renewcommand{\angle}[1]{\ensuremath{\mathrm{A}\left(#1 \right)}}
\newcommand{\axis}[1]{\ensuremath{\mathrm{V}\left(#1 \right)}}
\newcommand{\vecop}{\ensuremath{\mathrm{V}_\mathrm{Q}}}
\newcommand{\quatop}{\ensuremath{\mathrm{Q}_\mathrm{v}}}
\newcommand{\jone}{\ensuremath{\mathrm{J}_\mathrm{1}}}
\newcommand{\jtwo}{\ensuremath{\mathrm{J}_\mathrm{2}}}
%% Symbols
\newcommand{\seg}[1]{{\ensuremath{\mathcal{B}_\mathrm{#1}}}}
\newcommand{\imu}[1]{{\ensuremath{\mathcal{S}_\mathrm{#1}}}}
\newcommand{\earth}[1]{{\ensuremath{\mathcal{E}_\mathrm{#1}}}}
\newcommand{\earthhat}[1]{{\ensuremath{\tilde{\mathcal{E}_\mathrm{#1}}}}}
\newcommand{\finger}[1]{{\ensuremath{\mathcal{F}_\mathrm{#1}}}}
\newcommand{\joint}[2]{{\ensuremath{\mathcal{J}_\mathrm{#1,#2}}}}
\newcommand{\chain}[1]{{\ensuremath{\mathcal{C}_\mathrm{#1}}}}

\newcommand{\test}[2]{\ensuremath{\mathcal{J}_{\mathrm{#1}\ifthenelse{\isempty{#2}{}}{}{,\mathrm{#2}}}}} \renewcommand{\joint}[2]{\ensuremath{\mathcal{J}_{\mathrm{#1}\ifthenelse{\isempty{#2}{}}{}{,\mathrm{#2}}}}}

\newcommand{\dof}[1]{\ensuremath{\mathrm{dof(\,#1\,)}}}
%% Special Quaternions
\newcommand{\quatimuseg}[3][]{\quat[#1]{\imu{#2}}{\seg{#3}}}
\newcommand{\quatimuimu}[3][]{\quat[#1]{\imu{#2}}{\imu{#3}}}
\newcommand{\quatimuearth}[3][]{\quat[#1]{\imu{#2}}{\earth{#3}}}
\newcommand{\quatsegseg}[3][]{\quat[#1]{\seg{#2}}{\seg{#3}}}
\newcommand{\quatsegimu}[3][]{\quat[#1]{\seg{#2}}{\imu{#3}}}
\newcommand{\quatsegearth}[3][]{\quat[#1]{\seg{#2}}{\earth{#3}}}
\newcommand{\quatearthseg}[3][]{\quat[#1]{\earth{#2}}{\seg{#3}}}
\newcommand{\quatearthimu}[3][]{\quat[#1]{\earth{#2}}{\imu{#3}}}
\newcommand{\quatearthearth}[3][]{\quat[#1]{\earth{#2}}{\earth{#3}}}

\newcommand{\quatsegimushift}[3][]{\quattilde[#1]{\seg{#2}}{\imu{#3}}}
\newcommand{\quatearthearthest}[3][]{\quatest[#1]{\earth{#2}}{\earth{#3}}}
\newcommand{\quatsegearthest}[3][]{\quatest[#1]{\seg{#2}}{\earth{#3}}}
\newcommand{\quatsegsegest}[3][]{\quatest[#1]{\seg{#2}}{\seg{#3}}}
%% Eulerangles
\newcommand{\eulere}[3]{\ensuremath{#1\text{-}#2\text{-}#3}}
\newcommand{\euleri}[3]{\ensuremath{#1\text{-}#2'\text{-}#3''}}

\newcommand{\alphahat}{\ensuremath{\hat{\alpha}} }
\newcommand{\betahat}{\ensuremath{\hat{\beta}} }
\newcommand{\gammahat}{\ensuremath{\hat{\gamma}} }

%% Special math operators
\newcommand{\norm}[1]{\ensuremath{\left\lVert#1\right\rVert}}
\newcommand{\normalized}[1]{\ensuremath{\frac{#1}{\norm{#1}}}}
\newcommand{\partialfrac}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\DeclareMathOperator{\atantwo}{atan2}
\newcommand{\argmin}[1]{\ensuremath{\underset{#1}{\operatorname{arg\,min}}}}

\newcommand{\f}{\ensuremath{\mathrm{f}}}
\renewcommand{\r}{\ensuremath{\mathrm{r}}}
%% Master thesis specific stuff
\newcommand{\he}{\ensuremath{\delta}}
\newcommand{\heest}{\ensuremath{\hat\delta}}
\newcommand{\het}{\ensuremath{\delta(t)}}
\newcommand{\heestt}{\ensuremath{\hat\delta(t)}}
\newcommand{\hef}{\ensuremath{\hat{\delta}_\mathrm{f}}}
\newcommand{\heft}{\ensuremath{\hat{\delta}_\mathrm{f}(t)}}
\newcommand{\heref}{\ensuremath{\delta_{\textrm{ref}}}}
\newcommand{\hereft}{\ensuremath{\delta_{\textrm{ref}}(t)}}
\newcommand{\hefw}{\ensuremath{\hat{\delta}_{\mathrm{f,}w}}}
\newcommand{\hefwm}{\ensuremath{\hat{\delta}_{\mathrm{f,}w-1}}}
\newcommand{\kdeltaw}{\ensuremath{k_{\he,w}}}
\newcommand{\kbiasw}{\ensuremath{k_{\mathrm{b,}w}}}

\newcommand{\mphase}[1]{M#1}
\newcommand{\rating}{\ensuremath{r}}
\newcommand{\ratingth}{\ensuremath{\rating_\mathrm{min}}}
\newcommand{\set}[2][]{\ensuremath{\mathrm{#2}_{\mathrm{#1}}}}

\newcommand{\req}[1]{\textbf{#1}}
\newcommand{\s}{\ensuremath{\,\mathrm{s}}}
\newcommand{\mm}{\ensuremath{\,\mathrm{mm}}}
\newcommand{\gs}{\ensuremath{^\circ/\mathrm{s}}}
\newcommand{\g}{\ensuremath{^\circ}}

\renewcommand{\i}{\ensuremath{\mathrm{i}}}
\newcommand{\p}{\ensuremath{\mathrm{p}}}
\newcommand{\dif}{\ensuremath{\mathrm{d}\!}}
\newcommand{\upquote}{\hspace{-0.2em}\textquotesingle}
\newcommand{\windowidx}{w}
\newcommand{\sampleidx}{k}
\newcommand{\TEst}{\ensuremath{T_\mathrm{est}}}
\newcommand{\TSet}{\ensuremath{T_\mathrm{set}}}
\newcommand{\TSample}{\ensuremath{T_\mathrm{s}}}
\newcommand{\TStill}{\ensuremath{T_\mathrm{St}}}
\newcommand{\NStill}{\ensuremath{N_\mathrm{St}}}
\newcommand{\OStill}{\ensuremath{\omega_\mathrm{St}}}
\newcommand{\TWin}{\ensuremath{T_\mathrm{w}}}
\newcommand{\TWinadapt}{\ensuremath{\tilde{T}_\mathrm{w}}}
\newcommand{\windowvar}[2][\windowidx]{\ensuremath{#2_{#1}}}
% \newcommand{\samplevar}[2][\sampleidx]{\ensuremath{#2_{\windowidx,#1}}}

\newcommand{\samplevar}[2][\sampleidx]{\ensuremath{#2_{#1}}}

\newcommand{\sample}[1]{\ensuremath{#1_{\sampleidx}}}
\newcommand{\windowsize}{\ensuremath{N_\textrm{w}}}
\newcommand{\te}{\ensuremath{{\epsilon_\mathrm{\scriptscriptstyle  RMS}}}}
\newcommand{\de}{\ensuremath{{\epsilon_{\delta,\mathrm{\scriptscriptstyle RMS}}}}}
\newcommand{\ehe}{\ensuremath{{\epsilon_{\delta}}}}
\newcommand{\ess}{\ensuremath{\epsilon_\mathrm{ss}}}
\newcommand{\eo}{\ensuremath{\earth{\mathrm{opt}}}}
\newcommand{\id}[2]{\ensuremath{#1\mathrm{D}\_0#2}}
\newcommand{\hid}[1]{\ensuremath{\mathrm{H}\_0#1}}

\newcommand{\sz}[1]{\scriptsize{#1}}

\newcommand{\windowN}{\ensuremath{N}}
\newcommand{\winduration}{\ensuremath{T_{\mathrm{win}}}}
\newcommand{\betaz}{\ensuremath{\beta_0}}
\newcommand{\betazest}{\ensuremath{\hat{\beta}_0}}
\newcommand{\seglen}[1]{\ensuremath{l_\mathrm{#1}}}

\newcommand{\squatimuseg}[3][]{\squat[#1]{\imu{#2}}{\seg{#3}}}
\newcommand{\squatimuimu}[3][]{\squat[#1]{\imu{#2}}{\imu{#3}}}
\newcommand{\squatimuearth}[3][]{\squat[#1]{\imu{#2}}{\earth{#3}}}
\newcommand{\squatsegseg}[3][]{\squat[#1]{\seg{#2}}{\seg{#3}}}
\newcommand{\squatsegimu}[3][]{\squat[#1]{\seg{#2}}{\imu{#3}}}
\newcommand{\squatsegearth}[3][]{\squat[#1]{\seg{#2}}{\earth{#3}}}
\newcommand{\squatearthseg}[3][]{\squat[#1]{\earth{#2}}{\seg{#3}}}
\newcommand{\squatearthimu}[3][]{\squat[#1]{\earth{#2}}{\imu{#3}}}
\newcommand{\squatearthearth}[3][]{\squat[#1]{\earth{#2}}{\earth{#3}}}







\newcommand{\n}[2][$\bullet$]{\par\setlength{\hangindent}{\widthof{#1 }}\hangafter0\noindent\llap{#1 }#2}

% % https://tex.stackexchange.com/questions/352580/package-color-error-argument-1-01125-no-in-range-0-1
% \makeatletter
% \p@=1pt
% \makeatother

\definecolor{C0}{HTML}{1F77B4}\definecolor{C0dark}{HTML}{195F90}\definecolor{C0dark2}{HTML}{103C5A}\definecolor{C0light}{HTML}{258FD8}\definecolor{C0light2}{HTML}{2CA9FF}
\definecolor{C1}{HTML}{FF7F0E}\definecolor{C1dark}{HTML}{CC660B}\definecolor{C1dark2}{HTML}{804007}\definecolor{C1light}{HTML}{FF7F0E}\definecolor{C1light2}{HTML}{FF7F0E}
\definecolor{C2}{HTML}{2CA02C}\definecolor{C2dark}{HTML}{238023}\definecolor{C2dark2}{HTML}{165016}\definecolor{C2light}{HTML}{35C035}\definecolor{C2light2}{HTML}{42F042}
\definecolor{C3}{HTML}{D62728}\definecolor{C3dark}{HTML}{AB1F20}\definecolor{C3dark2}{HTML}{6B1314}\definecolor{C3light}{HTML}{FF2E30}\definecolor{C3light2}{HTML}{FF2E30}
\definecolor{C4}{HTML}{9467BD}\definecolor{C4dark}{HTML}{765297}\definecolor{C4dark2}{HTML}{4A335E}\definecolor{C4light}{HTML}{B27CE3}\definecolor{C4light2}{HTML}{C88BFF}
\definecolor{C5}{HTML}{8C564B}\definecolor{C5dark}{HTML}{70453C}\definecolor{C5dark2}{HTML}{462B26}\definecolor{C5light}{HTML}{A8675A}\definecolor{C5light2}{HTML}{D28171}
\definecolor{C6}{HTML}{E377C2}\definecolor{C6dark}{HTML}{B65F9B}\definecolor{C6dark2}{HTML}{723C61}\definecolor{C6light}{HTML}{FF86DA}\definecolor{C6light2}{HTML}{FF86DA}
\definecolor{C7}{HTML}{7F7F7F}\definecolor{C7dark}{HTML}{666666}\definecolor{C7dark2}{HTML}{404040}\definecolor{C7light}{HTML}{989898}\definecolor{C7light2}{HTML}{BEBEBE}
\definecolor{C8}{HTML}{BCBD22}\definecolor{C8dark}{HTML}{96971B}\definecolor{C8dark2}{HTML}{5E5E11}\definecolor{C8light}{HTML}{E2E329}\definecolor{C8light2}{HTML}{FEFF2E}
\definecolor{C9}{HTML}{17BECF}\definecolor{C9dark}{HTML}{1298A6}\definecolor{C9dark2}{HTML}{0C5F68}\definecolor{C9light}{HTML}{1CE4F8}\definecolor{C9light2}{HTML}{1CEAFF}
\newcommand{\old}[1]{\textcolor{C1}{#1}}
\newcommand{\red}[1]{\textcolor{C3}{#1}}


\newcommand{\sumphantom}{\left(\sum_{i+10}^{p+12} \right)}
\ExplSyntaxOn

\NewDocumentCommand \inlinevec { s o m }
 {
  \IfBooleanTF {#1}
   { \vectaux*{#3} }
   { \IfValueTF {#2} { \vectaux[#2]{#3} } { \vectaux{#3} } }
  ^\mathrm{T}
 }

\NewDocumentCommand \inlinerowvec { s o m }
 {
  \IfBooleanTF {#1}
   { \vectaux*{#3} }
   { \IfValueTF {#2} { \vectaux[#2]{#3} } { \vectaux{#3} } }
 }

\DeclarePairedDelimiterX \vectaux [1] {\lbrack} {\rbrack}
 { \, \dbacc_vect:n { #1 } \, }

\cs_new_protected:Npn \dbacc_vect:n #1
 {
  \seq_set_split:Nnn \l_tmpa_seq { , } { #1 }
  \seq_use:Nn \l_tmpa_seq { \enspace }
 }
\ExplSyntaxOff
